Traceable Group-Wise Self-Optimizing Feature Transformation Learning: A Dual Optimization Perspective

Feature transformation aims to reconstruct an effective representation space by mathematically refining the existing features. It serves as a pivotal approach to combat the curse of dimensionality, enhance model generalization, mitigate data sparsity, and extend the applicability of classical models. Existing research predominantly focuses on domain knowledge-based feature engineering or learning latent representations. However, these methods, while insightful, lack full automation and fail to yield a traceable and optimal representation space. An indispensable question arises: Can we concurrently address these limitations when reconstructing a feature space for a machine-learning task? Our initial work took a pioneering step towards this challenge by introducing a novel self-optimizing framework. This framework leverages the power of three cascading reinforced agents to automatically select candidate features and operations for generating improved feature transformation combinations. Despite the impressive strides made, there was room for enhancing its effectiveness and generalization capability. In this extended journal version, we advance our initial work from two distinct yet interconnected perspectives: 1) We propose a refinement of the original framework, which integrates a graph-based state representation method to capture the feature interactions more effectively and develop different Q-learning strategies to alleviate Q-value overestimation further. 2) We utilize a new optimization technique (actor-critic) to train the entire self-optimizing framework in order to accelerate the model convergence and improve the feature transformation performance. Finally, to validate the improved effectiveness and generalization capability of our framework, we perform extensive experiments and conduct comprehensive analyses.

==> abstract.tex <==
\begin{abstract}
Feature transformation aims to extract a good representation (feature) space by mathematically transforming existing features. 
It is crucial to address the curse of dimensionality, enhance model generalization, overcome data sparsity, and expand the availability of classic models. Current research focuses on domain knowledge-based feature engineering or learning latent representations; nevertheless, these methods are not entirely automated and cannot produce a traceable and optimal representation space. When rebuilding a feature space for a machine learning task, can these limitations be addressed concurrently?
To achieve this goal, we propose a novel self-optimizing framework that employs three cascading reinforced agents to automatically select candidate features and operations for better feature transformation.
In the preliminary work, we present a self-optimizing framework for feature transformation that employs three cascading reinforced agents to learn effective policies for selecting candidate features and operations for feature crossing.
While it has achieved good performance, the effectiveness of the reconstructed feature space can be improved by: (1) obtaining an advanced state representation for enabling reinforced agents to comprehend the current feature set better; and (2) resolving Q-value overestimation in reinforced agents for learning unbiased and effective policies.
Thus, in the journal version, to fulfill goal 1, 
it is assumed that an effective state representation should not only contain the entire feature set knowledge, but also capture feature-feature correlations.
First, we build a complete graph based on feature-feature correlations.
Then, using  message-passing,  we aggregate feature knowledge based on the learned graph structure to obtain a graph embedding.
The graph embedding can recover the original graph, which is the state representation. 
To fulfill goal 2, we undertake Q-learning using two Q-networks: one for action selection  and the other for Q-value estimation.  We divide the learning process in each Q-Network into two streams: state value estimation and action advantage value estimation. The Q-value is the combination of the two streams' estimations. 
Finally, to make experiments more convincing than the preliminary work, we conclude by adding the outlier detection task with five datasets, evaluating various state representation approaches, and comparing different training strategies. Extensive experiments and case studies show that our work is more effective and superior.
\end{abstract}

==> bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/mengxiao.jpg}}]{Meng Xiao}
was born in 1995. He received his B.S. degree from the East China University of Technology and graduated from China University of Geosciences (Wuhan) with a master's degree. He is currently working toward obtaining a Ph.D. degree at the University of Chinese Academy of Sciences. His main research interests include Data Mining, Graph Representation Learning, and Reinforcement Learning.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/dongjie.jpeg}}]
{Dongjie Wang}
 received the BE degree from
the Sichuan University, China, 2016, the MS degree from the Southwest Jiaotong University, China, 2017. He is currently working toward the PhD degree at the University of Central Florida (UCF). His research
interests include Anomaly Detection, Generative Adversarial Network, Reinforcement Learning and Spatio-temporal Data Mining.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/yanjie.jpeg}}]{Yanjie Fu}
is an Assistant Professor in the Department of Computer Science at the University of Central Florida. He received his Ph.D. degree from Rutgers, the State University of New Jersey in 2016, the B.E. degree from University of Science and Technology of China in 2008, and the M.E. degree from Chinese Academy of Sciences in 2011. His research interests include Data Mining and Big Data Analytics.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/kunpeng_liu.pdf}}]
{Kunpeng Liu} is an Assistant Professor in the Department of Computer Science, Portland State University. Prior to that, he received the Ph.D. degree from the CS Department of the University of Central Florida. He received both his M.E. degree and B.E. degree from the Department of Automation, University of Science and Technology of China (USTC). He has rich research experience in industry research labs, such as Geisinger Medical Research, Microsoft Research Asia, and Nokia Bell Labs. He has published in refereed journals and conference proceedings, such as IEEE TKDE, ACM SIGKDD, IEEE ICDM, AAAI, and IJCAI. He has received a Best Paper Runner-up Award from IEEE ICDM 2021.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/minwu.jpeg}}]{Min Wu}
Min Wu is currently a Senior Scientist in Machine Intellection Department, Institute for Infocomm Research, Agency for Science, Technology and Research (A*STAR), Singapore. He received his Ph.D. degree in Computer Science from Nanyang Technological University (NTU), Singapore, in 2011 and B.S. degree in Computer Science from University of Science and Technology of China (USTC) in 2006. He received the best paper awards in InCoB 2016 and DASFAA 2015, and the finalist academic paper award in IEEE PHM 2020. He also won the CVPR UG2+ challenge in 2021 and the IJCAI competition on repeated buyers prediction in 2015. His current research interests include machine learning, data mining and bioinformatics.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/huixiong.jpg}}]{Hui Xiong}
 is currently a Chair Professor at the
Hong Kong University of Science and Technol-
ogy (Guangzhou). Dr. Xiong’s research interests
include data mining, mobile computing, and their
applications in business. Dr. Xiong received his
PhD in Computer Science from University of
Minnesota, USA. He has served regularly on the
organization and program committees of numer-
ous conferences, including as a Program Co-
Chair of the Industrial and Government Track for
the 18th ACM SIGKDD International Conference
on Knowledge Discovery and Data Mining (KDD), a Program Co-Chair
for the IEEE 2013 International Conference on Data Mining (ICDM), a
General Co-Chair for the 2015 IEEE International Conference on Data
Mining (ICDM), and a Program Co-Chair of the Research Track for the
2018 ACM SIGKDD International Conference on Knowledge Discovery
and Data Mining. He received the 2021 AAAI Best Paper Award and
the 2011 IEEE ICDM Best Research Paper award. For his outstanding
contributions to data mining and mobile computing, he was elected an
AAAS Fellow and an IEEE Fellow in 2020.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/yuanchunzhou.jpg}}]{Yuanchun Zhou}
was born in 1975. He received his Ph.D. degree from Institute of Computing Technology, Chinese Academy of Sciences, in 2006. He is a Professor, Ph.D. supervisor, and the Assistant Director of Computer Network Information Center, Chinese Academy of Sciences, as well as the Director of the Department of Big Data Technology and Application Development. His research interests include data mining, big data processing, and knowledge graph.
\end{IEEEbiography}

